Detect to Learn: Structure Learning with Attention and Decision Feedback for MIMO-OFDM Receive Processing

The limited over-the-air (OTA) pilot symbols in multiple-input-multiple-output orthogonal-frequency-division-multiplexing (MIMO-OFDM) systems presents a major challenge for detecting transmitted data symbols at the receiver, especially for machine learning-based approaches. While it is crucial to explore effective ways to exploit pilots, one can also take advantage of the data symbols to improve detection performance. Thus, this paper introduces an online attention-based approach, namely RC-AttStructNet-DF, that can efficiently utilize pilot symbols and be dynamically updated with the detected payload data using the decision feedback (DF) mechanism. Reservoir computing (RC) is employed in the time domain network to facilitate efficient online training. The frequency domain network adopts the novel 2D multi-head attention (MHA) module to capture the time and frequency correlations, and the structural-based StructNet to facilitate the DF mechanism. The attention loss is designed to learn the frequency domain network. The DF mechanism further enhances detection performance by dynamically tracking the channel changes through detected data symbols. The effectiveness of the RC-AttStructNet-DF approach is demonstrated through extensive experiments in MIMO-OFDM and massive MIMO-OFDM systems with different modulation orders and under various scenarios.

==> algorithm/alg_sym_detect_procedure.tex <==
\begin{algorithm}
\caption{Symbol Detection Procedure of RC-AttStructNet-DF}\label{alg:rc_structnet_df}
\scriptsize
% \tiny
\begin{algorithmic}[1]
    \commentline{Offline initialization}
    \State Prepare artificial training data
    \State Train a binary classifier with artificial training data
    \State Initialize binary classifier in StructNet with learned weights
    \commentline{Online training}
    \For{Each OFDM subframe}
        \commentline{Learning from pilot symbols}
        \State \multiline{Prepare pilot training data $D_{rc}$ with time domain received and transmitted pilot signals as defined in eq.~(\ref{eq:rc_pilot_train_data})}
        \State \multiline{Train output weights of RC with $D_{rc}$ using one-shot LS solution in eq.~(\ref{equ:rc_least_square})}
        \State \multiline{Generate RC output (time domain RC pilot output) when tested on received pilot signals}
        \State Transform time domain RC pilot output to frequency domain (frequency domain RC pilot output) 
        \State Utilize frequency domain RC pilot output and transmitted pilot symbols to estimate effective channel using LMMSE
        \State Initialize PE layer of StructNet with estimated effective channel
        \State Prepare pilot training data for 2D MHA and StructNet with frequency domain RC pilot output and transmitted pilot symbols
        \State Train 2D MHA and StuctNet with pilot training data using attention loss
        \commentline{DF with data symbols}
        \For{OFDM symbol $n = N_p: N-1$ (data symbols)}
            \State Generate RC output ($n$-th time domain RC data output) by testing on $n$-th time domain received data signal
            \State Prepare training dataset for RC with $n$-th time domain received data signal and $n$-th time domain RC data output
            \State Update RC weights by RLS algorithm following eq.~(\ref{eq:rls_weight_update})
            \State Transform $n$-th time domain RC data output to frequency domain ($n$-th frequency domain RC data output)
            \If{$n=N_p$}
                \State \multiline{Generate $n$-th detected data symbols with 2D MHA and StructNet by testing on $n$-th frequency domain RC data output}
            \Else
                \State \multiline{Generate $n$-th detected data symbols with StructNet by testing on $n$-th frequency domain RC data output}
            \EndIf
            \State \multiline{Prepare training dataset for StructNet with $n$-th frequency domain RC data output and $n$-th detected data symbols }    
            \State Fine-tune StructNet weights with attention loss
        \EndFor
    \EndFor
\end{algorithmic}
\end{algorithm}
